Test-Time Alignment for Tracking User Interest Shifts in Sequential Recommendation

Sequential recommendation is essential in modern recommender systems, aiming to predict the next item a user may interact with based on their historical behaviors. However, real-world scenarios are often dynamic and subject to shifts in user interests. Conventional sequential recommendation models are typically trained on static historical data, limiting their ability to adapt to such shifts and resulting in significant performance degradation during testing. Recently, Test-Time Training (TTT) has emerged as a promising paradigm, enabling pre-trained models to dynamically adapt to test data by leveraging unlabeled examples during testing. However, applying TTT to effectively track and address user interest shifts in recommender systems remains an open and challenging problem. Key challenges include how to capture temporal information effectively and explicitly identifying shifts in user interests during the testing phase. To address these issues, we propose T$^2$ARec, a novel model leveraging state space model for TTT by introducing two Test-Time Alignment modules tailored for sequential recommendation, effectively capturing the distribution shifts in user interest patterns over time. Specifically, T$^2$ARec aligns absolute time intervals with model-adaptive learning intervals to capture temporal dynamics and introduce an interest state alignment mechanism to effectively and explicitly identify the user interest shifts with theoretical guarantees. These two alignment modules enable efficient and incremental updates to model parameters in a self-supervised manner during testing, enhancing predictions for online recommendation. Extensive evaluations on three benchmark datasets demonstrate that T$^2$ARec achieves state-of-the-art performance and robustly mitigates the challenges posed by user interest shifts.

==> sections/0_abstract.tex <==
\begin{abstract}
Sequential recommendation is essential in modern recommender systems, aiming to predict the next item a user may interact with based on their historical behaviors. However, real-world scenarios often present challenges related to distribution shifts. Existing methods are typically trained on static historical data and struggle to effectively adapt to these changes, leading to significant performance degradation. To address this challenge, Test-Time Training (TTT) has emerged as a promising new paradigm, enabling pre-trained models to dynamically adapt to test data by leveraging unlabeled samples during inference for self-adaptation. However, existing works mainly focus on adapting to shifts in data features, overlooking the changes in user interest patterns at the test time. To address this issue, we propose \textbf{\ourname}, a novel model that integrates \textbf{TTT} into sequential recommendation by introducing two \textbf{A}lignment-based self-supervised losses, effectively capturing the distribution shifts in user interest patterns over time. By continuously updating model parameters during inference, \ourname\ adapts to test-time data, significantly improving performance. Specifically, we align absolute time intervals with model-adaptive learning intervals to better capture temporal dynamics and introduce a \oursslname\ alignment mechanism to more effectively understand the current user interest pattern. These two alignment-based self-supervised losses are used to optimize predictions during inference. Extensive evaluations on three benchmark datasets demonstrate that \ourname\ achieves state-of-the-art performance and robustly mitigates the challenges posed by data distribution shifts. Our source code is available at \url{https://github.com/lyingCS/OurName}.
\end{abstract}


==> sections/1_intro.tex <==
\section{Introduction}
% Recommender systems, as a crucial branch of data mining, provide essential and powerful solutions for alleviating information overload and enhancing user experiences~\cite{qu2023continuous, qu2024budgeted, qu2024scalable}. In recent years, numerous recommendation algorithms have been proposed, including sequential recommendation~\cite{zhang2024reinforcing}, graph-based recommendation~\cite{zhang2024qagcf}, and cross-domain recommendation~\cite{zhang2024modeling}. Sequential recommendation systems aim to predict the next item a user will interact with by modeling dependencies within their historical interaction data. 

\begin{figure}[t]
\centering
\includegraphics[width=0.45 \textwidth]{fig/intro.png}
\caption{Illustrates of user interest shifts between train and test phases in sequential recommendation. During the Train Phase (weekdays), the user’s historical behavior is focused on study-related content (e.g., books), and the model learns to predict the next item based on this pattern. In the Test Phase (weekends), user interests shift from study-related items to leisure activities (e.g., sports). Although the Test input includes the ground truth from the Train Phase, the model continues to recommend study-related content, failing to adapt to the user’s new preferences. This highlights the importance of modeling temporal contexts and handling user interest shifts effectively in recommendations.}
\label{intro}
\end{figure}



Sequential recommendations aim to predict the next item a user will interact with by modeling dependencies within their historical interaction data~\cite{tang2018personalized, hidasi2015session, sun2019bert4rec, kang2018self,liu2024mamba4rec, xie2022contrastive, chang2021sequential, zhang2024reinforcing, fang2020deep, dai2024recode, zhang2024saqrec}. However, real-world scenarios often present the challenge of distribution shifts, where user behavior patterns and data distributions evolve dynamically over time. Existing methods, typically trained on static historical data, struggle to adapt to these changes, resulting in significant performance degradation~\cite{yang2024dual, sun2020test, liang2024comprehensive}. To address this issue, Test-Time Training (TTT) has emerged as a promising paradigm~\cite{liu2021ttt++, jin2022empowering, wang2022test, sun2020test, liang2024comprehensive}. TTT enables pre-trained models to dynamically adapt to test data by leveraging unlabeled samples during inference, allowing the model to achieve self-adaptation and effectively handle evolving distribution shifts. Recently, some works have applied TTT to recommendations~\cite{yang2024dual, yang2024ttt4rec, wang2024not}, yielding significant online benefits~\cite{wang2024not}.

However, we argue that existing work has not fully addressed the problem of distribution shift in recommendations. Distribution shift refers to the change in the joint distribution of inputs $X$ and outputs $Y$, i.e., $P_t(X, Y)$, over time. Notably, $P_t(X, Y)$ can be factorized as $P_t(X) \times P_t(Y|X)$. While existing approaches have primarily leveraged Test-Time Training to adapt to shifts in $P_t(X)$, such as changes in user or item features~\cite{yang2024dual}, no work has explored how to adapt to scenarios where $P_t(Y|X)$ changes at the test time. In sequential recommendation, this specifically reflects shifts in user interest patterns, where the next interaction target $Y$ may evolve over time even for the same user behavior sequence $X$.

\begin{figure}[t]
\centering
\includegraphics[width=0.45 \textwidth]{fig/combined.png}
\caption{Illustrates of users' interest shifts.}
\label{vali}
\end{figure}

For instance, consider a sequential recommendation where a user’s interaction history (as shown in Figure~\ref{intro}) during the train phase (weekdays) exhibits a strong preference for study-related items, such as books, reflecting their focus on work or learning. However, during the test phase (weekends), the user’s interest shifts towards sports-related items, such as football or basketball equipment, as they transition to leisure activities. If the recommendation fails to adapt to this shift and continues to recommend study-related items based on the Train Phase, it will not align with the user’s weekend preferences. This example illustrates how user behavior evolves dynamically between the training and testing phases, driven by contextual factors such as time availability and changing priorities, necessitating adaptive models to handle such user interest shifts effectively.

Based on these findings, we believe that solving this issue hinges on two key aspects: first, capturing temporal information, as user behavior are often influenced by periodic patterns or trending topics, making it crucial to understand the impact of historical events on predictions at specific future time points; second, dynamically adjusting the representation of user interest patterns, since even if a user’s historical behavioral features remain stable, their interest patterns may evolve dynamically. The model needs to identify and adapt to these changes in a timely manner to provide more accurate recommendations.

To address user interest shifts at the test time in sequential recommendation tasks, we propose \ourname, a sequential model based on Test-Time Training. \ourname\ introduces two alignment-based self-supervised losses to adaptively capture these shifts. The time interval alignment loss computes differences between interaction intervals in the sequence and the target prediction time, aligning these intervals with adaptive time steps to effectively capture temporal dynamics. The \oursslname\ alignment loss models the dynamic evolution of user interest patterns by transforming the input sequence into a final state, applying forward and backward state updates to generate a reconstructed state, and aligning it with the original state for precise pattern modeling. To address test-time throughput concerns, our model \ourname\ adopts Mamba-2~\cite{gu2023mamba, dao2024transformers} as the backbone, replacing the Transformer architecture's quadratic complexity with respect to sequence length~\cite{kang2018self}. During testing, \ourname\ applies gradient descent on test data to adjust model parameters in real time, enabling accurate next-item predictions under distribution shifts. This design allows \ourname\ to effectively capture temporal dynamics and adapt to evolving user interest patterns, ensuring robust and efficient performance in sequential recommendation tasks at the test time.

% To implement these ideas, we enhance the Mamba module~\cite{gu2023mamba, dao2024transformers}, known for its ability to handle long sequences, to create \ourblockname\ Block. By integrating \ourblockname\ into \ourname, the model dynamically adapts to test-phase data using the proposed alignment losses.

Our main contributions are as follows:
\begin{itemize}[leftmargin=*]
    \item Identification of a key issue in applying Test-Time Training to sequential recommendations: The overlooked shift in the user interest pattern $P_t(Y|X)$ at the test time.
    \item Introduction of a novel approach: We propose \ourname, a TTT-based sequential recommendation model incorporating two alignment-based self-supervised losses to capture temporal dynamics and evolving user interest patterns, along with real-time parameter adjustment during testing to address user interest shifts and ensure robust performance.
    \item Extensive experiments: We conduct experiments on three widely used datasets, demonstrating the effectiveness of \ourname. Further ablation studies and analysis explain the superiority of our designed modules.
\end{itemize}

==> sections/2_related.tex <==
\section{Related Work}
\subsection{Sequential Recommendation}
Sequential recommendations have evolved from traditional models, like Markov Chains~\cite{he2016fusing}, to deep learning approaches. Early RNN-based models (e.g., GRU4Rec~\cite{hidasi2015session}, HRNN~\cite{quadrana2017personalizing}) addressed long-range dependencies, leveraging hidden states to capture dynamic user preferences. Recently, Transformer-based architectures, such as SASRec~\cite{kang2018self} and BERT4Rec~\cite{sun2019bert4rec}, have gained prominence with self-attention mechanisms that model complex interactions and enable efficient parallel computation. Alternative methods, like MLP-based models (e.g., FMLP-Rec~\cite{zhou2022filter}), offer a balance between accuracy and efficiency. Innovations like Mamba4Rec\cite{liu2024mamba4rec} further enhance performance on long interaction sequences, reflecting the ongoing advancements in this field.
\subsection{Test-Time Training}
Test-Time Training (TTT)~\cite{liu2021ttt++, jin2022empowering, wang2022test} is an approach designed to improve model generalization by enabling partial adaptation during the test phase to address distribution shifts between training and testing datasets. It leverages self-supervised learning (SSL)~\cite{liu2022graph, schiappa2023self, yang2024mixed, liu2021self} tasks to optimize a supervised loss (e.g., cross-entropy) and an auxiliary task loss during training, with the objective formulated as:
\begin{equation}
    \mathcal{L}_{\text{TTT}} = \mathcal{L}_{\text{sup}} + \mu \mathcal{L}_{\text{aux}},
\end{equation}
where \(\mathcal{L}_{\text{sup}}\) is the supervised loss, \(\mathcal{L}_{\text{aux}}\) is the auxiliary task loss, and \(\mu\) is a balancing hyperparameter. The auxiliary task (e.g., rotation prediction) allows the model to align test-time features closer to the source domain. Simplified approaches like Tent~\cite{wang2020tent} avoid supervised loss optimization during testing, while advanced methods such as TTT++~\cite{liu2021ttt++} and TTT-MAE~\cite{he2022masked} employ techniques like contrastive learning and masked autoencoding to enhance adaptation. Unsupervised extensions, such as ClusT3~\cite{hakim2023clust3}, use clustering with mutual information maximization but face limitations due to hyperparameter sensitivity. TTT has also been applied to out-of-distribution (OOD) tasks, including recommendations~\cite{yang2024dual, yang2024ttt4rec, wang2024not}, enabling dynamic adaptation to distribution shifts and improving performance while achieving stable online gains~\cite{wang2024not}.

==> sections/3.0_pr.tex <==
\section{Problem Formulation}
\subsection{Preliminaries}\label{seqrec}
In sequential recommendation, let \( U = \{ u_1, u_2, \dots, u_{|U|} \} \) denote the user set, \( V = \{ v_1, v_2, \dots, v_{|V|} \} \) denote the item set, and \( S_u = \{ (v_1, t_1), (v_2, t_2), \dots, (v_{n_u}, t_{n_u}) \} \) denote the chronologically ordered interaction sequence for user \( u \in U \), where \( n_u \) is the length of the sequence, \( v_i \) is the \( i \)-th item interacted with by user \( u \), and \( t_i \) is the timestamp of the interaction. In the following sections, we omit the subscript \(u\) in \(n_u\) and directly use \(n\) as indices for convenience. Given the interaction history \( S_u \) and the predicted timestamp \( t_{n+1} \), the task is to predict the next interacted item \( v_{n+1} \), i.e., the item that the user \( u \) is most likely to interact with at timestamp \( t_{n+1} \). This can be formalized as learning a function:
\begin{equation}
f_{t_{n+1}}(S_u) \rightarrow v_{n+1},    
\end{equation}
where \( f_{t_{n+1}} \) maps the historical sequence \( S_u \) at timestamp \( t_{n+1} \) to the next likely item \( v_{n+1} \) from the item set \( V \).

\subsection{Modeling via State Space Models}\label{mamba}
Despite Transformer architecture-based models achieving outstanding performance in sequential recommendation~\cite{kang2018self}, their quadratic computational complexity with respect to the sequence length hinders efficient training during the test phase, imposing a significant load on test-time throughput. To address this, our model \ourname\ adopts the Mamba-2~\cite{gu2023mamba, dao2024transformers} as our backbone, which is derived from State Space Models (SSMs).

SSMs are a sophisticated sequence modeling framework based on linear ordinary differential equations, efficiently mapping input \(x(t) \in \mathbb{R}\) to output \(y(t) \in \mathbb{R}\) at current time $t$ through a $d_s$-dimensional hidden state \(h(t) \in \mathbb{R}^{d_s}\). These models leverage the dynamics described below:
\begin{subequations}  
\begin{equation}  
h^{\prime}(t) = A h(t) + B x(t), \label{ssm1} 
\end{equation}  
\begin{equation}  
y(t) = C h(t) + D x(t). \label{ssm2}
\end{equation}  
\end{subequations}
where \(A \in \mathbb{R}^{d_s \times d_s}\) and \(B, C \in \mathbb{R}^{d_s \times 1}\) are adjustable matrices. To enable effective representation of discrete data, SSMs employ the Zero Order Hold (ZOH)~\cite{gu2021combining} method for data discretization based on a specified step size \(\Delta\):

\begin{equation}
\begin{aligned}
h(t) & =e^{\Delta A} h(t-1)+\int_{t-1}^t e^{A ( t - \tau )} B x(\tau) d \tau \\
& \approx e^{\Delta A} h(t-1)+\int_{t-1}^t e^{A(t-\tau)} d \tau B x(t) \\
& =e^{\Delta A} h(t-1)+(\Delta A)^{-1}\left(e^{\Delta A}-I\right) \Delta B x(t).
\end{aligned}
\label{des}
\end{equation}
This results in the formulas:
\begin{subequations}  
\begin{equation}  
h_t =\bar{A} h_{t-1}+\bar{B} x_t, \label{dssm1} 
\end{equation}  
\begin{equation}  
y_t =C h_t+D x_t. \label{dssm2}
\end{equation}  
\end{subequations}
where $\bar{A}=e^{\Delta A}$ and $\bar{B}=(\Delta A)^{-1}\left(e^{\Delta A}-I\right)\Delta B$.

SSMs excel in long-sequence modeling~\cite{liu2024mamba4rec}, image generation~\cite{xu2024survey}, and reinforcement learning~\cite{ota2024decision}, providing efficient autoregressive inference like Recurrent Neural Networks~\cite{lipton2015critical} while processing input sequences in parallel like Transformers~\cite{vaswani2017attention}. This dual functionality enables efficient training and robust performance in applications such as time series analysis~\cite{rangapuram2018deep} and audio generation~\cite{goel2022s}.

The introduction of the Mamba~\cite{gu2023mamba} model significantly enhances SSMs by dynamically adjusting the matrices \(A\), \(B\), \(C\) and the step size \(\Delta\) dynamically depending on inputs. Its latest version, Mamba-2~\cite{dao2024transformers}, links structured state space models with attention mechanisms. Mamba-2 refines \(A\) into a scalar-times-identity matrix, creating a new state space duality (SSD) framework with multi-head patterns akin to Transformers. This innovation boosts training speed and increases state size, optimizing expressiveness for greater efficiency and scalability, making it a strong contender in language modeling against Transformers.

==> sections/3_method.tex <==
\input{sections/3.0_pr}
\begin{figure}[t]
\centering
\includegraphics[width=0.48 \textwidth]{fig/main1.png}
\caption{Overall Framework of \ourname: \ourname\ processes input sequences through an embedding layer, followed by the \ourblockname\ Layer and \ourssmname\ for state updates and output generation. The prediction layer generates final output embedding $\mathbf{p}_n$ for next-item predictions. The final output embedding $\mathbf{p}_n$ is reintroduced into the \ourblockname\ Layer to compute the \oursslname\ alignment loss.}
\label{main_model1}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{fig/main2.png}
\caption{The loss computation in \ourname\ and the logic of \ourssmname: The left side illustrates the time interval alignment loss (\(\mathcal{L}_{\text{ssl1}}\)), which aligns the predicted time intervals \(\Delta\) with the ground truth \(T\). The right side shows the \oursslname\ alignment loss (\(\mathcal{L}_{\text{ssl2}}\)), aligning the final state \(h_n\) with the backward-computed state \(\hat{h}_n\). These two losses jointly enhance the model’s robustness and effectiveness in handling user interest shifts. During testing, the model leverages these self-supervised losses to perform gradient descent, adapting to the input data and improving prediction performance.}
\label{main_model2}
\end{figure*}
\section{\ourname: The Proposed Method}
\subsection{Overall Framework}\label{overall}
As illustrated in Figure~\ref{main_model1}, the sequence \( S \) first passes through a learnable embedding layer \( \mathbf{E} = \{\mathbf{e}_1, \mathbf{e}_2, \ldots, \mathbf{e}_{|V|}\} \in \mathbb{R}^{|V| \times d} \), where \( d \) denotes the embedding dimension. This layer transforms the sparse vector representation of items into dense vector representations, with \( \mathbf{e}_j \) representing the dense vector for item \( v_j \). The sequence then enters our core \ourblockname\ layer, implemented based on the Mamba-2 module~\cite{gu2023mamba, dao2024transformers} (detailed in Section~\ref{mamba}), which replaces Transformer-based models to improve test-time throughput. The sequence undergoes a series of transformations to generate inputs for \ourssmname. Specifically, it produces the input \( x \in \mathbb{R}^{n \times d} \) for state updates, along with learnable matrices \( A \in \mathbb{R}^{1} \), \( B \in \mathbb{R}^{n \times d_s} \), \( C \in \mathbb{R}^{n \times d_s} \) (where \( d_s \) denotes the state dimension), and \( \Delta \in \mathbb{R}^{n} \), consistent with the Mamba2~\cite{dao2024transformers} module. Additionally, it generates learnable matrices \( P \in \mathbb{R}^{n \times d_s} \), \( Q \in \mathbb{R}^{n \times d_s} \), and \( \Delta' \in \mathbb{R}^{n} \) for backward state computation.

Within \ourssmname, a sequence of computations is performed to produce the output \( y \in \mathbb{R}^{n\times d} \), which is then passed through a Feed Forward Network (FFN) layer to adapt the features to the semantic space of the next layer. This process involves residual connections, layer normalization, and other transformations while leveraging the input sequence's timestamps to construct the time interval alignment loss (detailed in Section~\ref{sslsec1}). Finally, the prediction layer generates the output \( \mathbf{p}_n \in \mathbb{R}^{d} \), which is used for next-item prediction. 

It is worth noting that after obtaining the final output \( \hat{p}_n \), it is reintroduced as input to the \ourblockname\ layer to establish the \oursslname\ alignment loss (detailed in Section~\ref{sslsec2}). During this process, the gradient computation for \( \mathbf{p}_n \) is stopped. 

\subsection{Time Interval Alignment}\label{sslsec1}
To more accurately capture the temporal information in distribution shifts, we introduce a time interval alignment loss in \ourname. As shown in the left half of Figure~\ref{main_model2}, we illustrate the computation method for the time interval alignment loss. Notice that in \ourssmname, the discretization process (as shown in Equation~(\ref{des})) involves the use of the time step $\Delta = \{\Delta_1, \Delta_2, \dots, \Delta_{n} \}$, where $\Delta_i \in \mathbb{R}^{1}$. Ensuring the correctness of the time step is crucial when addressing distribution shifts. A correct time step helps better capture the temporal information of distribution shifts. 

As discussed in Section~\ref{overall}, the time step $\Delta$ in the \ourblockname\ block is not fixed but is dynamically generated based on the current input. 
% Specifically, let the current input at time \(t\) be denoted as \(x_t\). The time step \(\Delta_t\) is computed as a function of the input, expressed as:
% \begin{equation}
% \Delta_t = f(x_t),
% \end{equation}
% where $\Delta_t\in \mathbb{R}^{1}$ and \(f(\cdot)\) is a learnable deep neural network that maps the input \(x_t\) to a corresponding time step \(\Delta_t\).
This dynamic adjustment allows the model to account for variations in input characteristics, leading to a more flexible temporal representation.

In the context of sequential recommendation (as described in Section~\ref{seqrec}), we can obtain the exact timestamps of the user $u$'s historical sequence $\{t_1, t_2, \dots, t_{n}\}$ and predict the next user's possible interactions at timestamp $t_{n+1}$. From these timestamps, we can compute the time interval sequence: 
\begin{equation}
T = \{t_2-t_1, t_3-t_2, \dots, t_{n+1}-t_{n}\},
\label{ti}
\end{equation}
where $T \in \mathbb{R}^{n}$, which can be regarded as the ground truth for time steps in $\Delta$ during the discretization process. 

Existing work directly uses this time interval sequence as $\Delta = \{\Delta_1, \Delta_2, \dots, \Delta_{n} \}$ to calculate the discretized matrix $\bar{A}$ and $\bar{B}$ in Equation~(\ref{dssm1}) and Equation~(\ref{dssm2})~\cite{fan2024tim4rec}. However, we believe that this approach has the following limitations in capturing specific time intervals:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Magnitude scaling issue}: These timestamps are typically recorded in Linux time format with millisecond-level precision. Directly using them in matrix computations leads to significant problems with scaling and alignment.
    \item \textbf{Data collection bias}: In practical offline recommendation datasets and online recommendations, the timestamps collected are sometimes not strictly accurate due to engineering reasons. This limitation arises from the data collection process, making it impossible to obtain absolutely precise timestamps of events.
\end{enumerate}
To address the above limitations, we propose using pairwise loss to mitigate these issues. Specifically, for the predicted time step sequence 
$\Delta = \{\Delta_1, \Delta_2, \dots, \Delta_{n}\}$
and the actual time interval sequence 
$T = \{T_1, T_2, \dots, T_{n}\},$ where $T_i = t_{i+1} - t_i$, 
we compute the pairwise self-supervise loss as follows:
\begin{equation}
\mathcal{L}_{\text{pairwise}} = \sum_{i < j} \max(0, 1 - (\Delta_i - \Delta_j) \cdot (T_i - T_j)),   
\end{equation}
where \((\Delta_i - \Delta_j)\) represents the predicted pairwise differences. \((T_i - T_j)\) represents the true pairwise differences. The loss penalizes mismatches between the relative signs of predicted and true differences, preserving the relative relationships between the time intervals instead of relying on their absolute values.

However, directly applying this loss introduces certain challenges. When handling long sequences (e.g., $50$–$200$ items), the computational complexity of pairwise difference calculations increases to \(O(n^2)\). To address this issue, we adopt a block-based computation approach to simplify the process. Specifically, the sequence is divided into smaller, non-overlapping blocks of size \(b\), and pairwise losses are computed independently within each block. For each block, we first calculate the pairwise differences for predicted values \((\Delta_i - \Delta_j)\) and ground truth values \((T_i - T_j)\). Next, we apply a mask to exclude invalid pairs, accommodating sequences of varying lengths. Finally, the loss for each block is computed using the hinge loss formulation and normalized by the total number of valid pairs across all blocks:
\begin{equation}
\mathcal{L_{\text{ssl1}}} = \frac{\sum_{\text{block}} \sum_{i < j} \max(0, 1 - (\Delta_i - \Delta_j) \cdot (T_i - T_j))}{\text{Total Valid Pairs}}.
\label{ssl1}
\end{equation}  
This approach reduces both computational and memory complexity from \(O(n^2)\) to \(O(b^2 \times \lceil n/b \rceil)\), significantly enhancing scalability for long sequences.

\subsection{User Interest State Alignment}\label{sslsec2}
To ensure the model accurately captures and represents the evolving patterns of user interests over time, we introduce a \oursslname\ alignment loss in \ourname. As shown in Figure~\ref{intro}, user interest shifts during testing often occur toward the end of the input sequence. Therefore, it is crucial for recommendation models to better understand and align with the user’s interests at the tail end. To achieve this, we align the final states of \ourblockname.

As illustrated on the right side of Figure~\ref{main_model2}, we present the computation process for the \oursslname\ alignment loss. First, we introduce a backward state update function, which is then applied to align the final state of the input user history sequence. Ensuring the correctness of the final states generated by the model is critical for addressing shifts in user interests.
\subsubsection{Backward State Update Function}
Given the forward state update function $h'(t) = A h(t) + B x(t)$ in Equation~(\ref{ssm1}), we derive its backward form as:
\begin{equation}
\begin{aligned}
h(t) &= A^{-1} h'(t) + \left( - A^{-1} B x(t) \right).
\end{aligned}
\end{equation}
To simplify the notation, we define:
\begin{equation}
\begin{aligned}
P = A^{-1}, \quad Q = -A^{-1} B.
\label{pq}
\end{aligned}
\end{equation}
Substituting these definitions, the backward state update function becomes:
\begin{equation}
h(t) = P h'(t) + Q x(t).
\end{equation}
For the discrete-time system, we adopt the Zero-Order Hold (ZOH)~\cite{gu2021combining} method and parameterize the system as follows:
\begin{equation}
\bar{P} = \exp(\Delta P), \quad \bar{Q} = (\Delta Q)^{-1}  \cdot (\exp(\Delta P) - I) \cdot \Delta Q,
\label{dispq}
\end{equation}
where $\Delta P$ and $\Delta Q$ are the continuous-time system matrices, and $\Delta$ denotes the discretization step size.

Using this parameterization, the backward discrete state update function can be expressed as:
\begin{equation}
\begin{aligned}
h_{t} &= \bar{P} h_{t+1} + \bar{Q} x_{t+1}.
\end{aligned}
\label{bds}
\end{equation}

\subsubsection{Interest State Alignment Loss}
For the current input sequence \(S = \{v_1, v_2, \dots, v_n\}\), given an all-zero matrix \(h_0\) as the initial state, the outputs \(y = \{y_1, y_2, \dots, y_n\}\) are generated according to Equation~(\ref{ssm1}) and Equation~(\ref{ssm2}). Meanwhile, the state transitions iteratively from \(h_0\) to \(h_1, h_2, \dots, h_n\), with \(h_n\) as the final state. At this point, we perform \oursslname\ alignment on \(h_n\).

Notice that \ourname's output embedding \(\hat{p}_n\) is compared with the embeddings of all items using a dot product to compute similarity, and the item with the highest similarity score is selected as the final prediction, which is detailed in Section~\ref{training}. Theoretically, the predicted \(y_n\) should approximate the next expected ground truth item \(v_{n+1}\). Based on this finding, we feed \(\hat{p}_{n}\) into the model to compute the input of the SSM as \(\hat{x}_{n+1}\), and \(\hat{h}_{n+1}\) can be estimated by performing a forward state update with \(h_n\) and \(\hat{x}_{n+1}\):
\begin{equation}
% h_{n+1} = \bar{A} h_n + \bar{B} v_{n+1} \approx \bar{A} h_n + \bar{B} y_n.
\hat{h}_{n+1} = \bar{A} h_n + \bar{B} \hat{x}_{n+1}.
\label{forward}
\end{equation}
Given \(\hat{h}_{n+1}\), we utilize the backward state update function to compute the backward state \(\hat{h}_n\), assessing the alignment between the original state \(h_n\) and the backward-computed state \(\hat{h}_n\). Specifically, as described in Section~\ref{overall} and illustrated in Figure~\ref{main_model1}, we take \(\hat{p}_n\) as input, passing it through a linear layer to output matrices \(P\), \(Q\), and \(\Delta'\). 
Notably, due to the definition of \(P\) and \(Q\) matrices in Equation~(\ref{pq}), we exclude non-linear activation layers to prevent the model from failing to learn the correct correspondence between \(P\), \(Q\), and \(A\), \(B\). Next, using Equation~(\ref{dispq}), we compute the discretized \(\bar{P}\) and \(\bar{Q}\), and finally, apply Equation~(\ref{bds}) to derive the following reconstructed final state:
\begin{equation}
% h_n = \bar{P} h_{n+1} + \bar{Q} x_{n+1}.
\hat{h}_n = \bar{P} \hat{h}_{n+1} + \bar{Q} \hat{x}_{n+1}.
\label{backward}
\end{equation}
Finally, we define the Interest State Alignment Loss as:
\begin{equation}
\mathcal{L}_{\mathrm{ssl} 2} = \left\|h_n - \hat{h}_n\right\|_2^2.
\label{ssl2}
\end{equation}
By reconstructing and aligning the final state of the current input sequence, the model can accurately understand the user interest pattern that evolves with the distribution shift.

\begin{algorithm}[tbp]
\caption{Test-Time Training for \ourname~ on a Single Batch}
\label{alg:test_time_training}
\raggedright
\textbf{Input:} Well-trained model \(g_\theta(\cdot)\), batch of test sequences \(S_{\text{test}}\) (size \(B\)), each represented as \(S^i_{\text{test}} = \{(v^i_1, t^i_1), (v^i_2, t^i_2), \dots, (v^i_n, t^i_n)\}\) with the corresponding prediction timestamp \(t^i_{n+1}\), number of training steps \(M\), learning rate \(\alpha\), and weight parameters \(\mu_1^{\text{test}}\) and \(\mu_2^{\text{test}}\).

\textbf{Output:} Final prediction \(\mathbf{p}_{\text{n}}\).

\begin{algorithmic}[1]
\STATE Record the original model parameters: \(\theta_{o} \gets \theta\).
\FOR{\(\text{step} = 1, 2, \ldots, M\)}
    \STATE Forward \(g_\theta(S_{\text{test}})\) and get the learned step size $\Delta$, final state \(h_n\) and output \(\mathbf{p}_n\).
    \STATE Compute the time interval sequence $T$ using Equation~(\ref{ti}).
    % using \(\{t_1, t_2, \cdots, t_{n+1}\}\)
    \STATE Calculate \(\mathcal{L}_{\text{ssl1}}\) from Equation~(\ref{ssl1}) using \(\Delta\) and $T$.
    \STATE Compute the forward state \(\hat{h}_{n+1}\) using Equation~(\ref{ssm1}). 
    % with \(h_n\) and \(y_n\).
    \STATE Compute the backward state \(\hat{h}_{n}\) using Equation~(\ref{backward}). 
    % with \(\hat{h}_{n+1}\) and \(y_n\).
    \STATE Calculate \(\mathcal{L}_{\text{ssl2}}\) from Equation~(\ref{ssl2}) using \(h_{n}\) and \(\hat{h}_{n}\).
    \STATE Update model parameters:
    \[
    \theta \gets \theta - \alpha \nabla_\theta \frac{1}{B} \left(\mu_1^{\text{test}}\mathcal{L}_{\text{ssl1}} + \mu_2^{\text{test}}\mathcal{L}_{\text{ssl2}}\right).
    \]
\ENDFOR
\STATE Compute the final prediction \(\mathbf{p}_{\text{n}}\) using the updated \(g_\theta(S_{\text{test}})\).
\STATE Restore the model parameters: \(\theta \gets \theta_{o}\) for the next batch.
\end{algorithmic}
\end{algorithm}

\subsection{Training and Testing Process}
\subsubsection{Training Process}\label{training}
After designing the two self-supervised losses, we compute the primary recommendation loss. Based on the embedding sequence generated by the previous layers, the prediction layer provides the final recommendation results. Specifically, the model uses the embedding of the last item in the sequence to predict the next item the user is likely to interact with.

Formally, let the sequence of item embeddings generated by the model be \({\mathbf{P}} = \{{\mathbf{p}}_1, {\mathbf{p}}_2, \dots, {\mathbf{p}}_{n}\}\in \mathbb{R}^{n\times d}\), where \({\mathbf{p}}_{n} \in \mathbb{R}^{d}\) represents the output embedding of the last item in the user’s interaction history. The prediction layer computes logits for all items in the item set as:
\begin{equation}
\hat{\mathbf{z}} = {\mathbf{p}_{n}} \mathbf{E}^\top,
\end{equation}
where $\mathbf{E}$ is the embedding table of the embedding layer.
The recommendation loss is then computed using the cross-entropy loss:
\begin{equation}
\mathcal{L}_{\text{rec}} = -\frac{1}{n} \sum_{i=1}^{n} z_i \log \left(\hat{z}_i\right)
\end{equation}
where $z_i$ denotes the ground-truth for item $i$, $\hat{z}_i$ denotes the predicted logit for item $i$ in $\mathbf{\hat{z}}$. This loss encourages the model to maximize the predicted probability of the true interacted item, improving recommendation accuracy.

Finally, the total loss of the model combines the primary recommendation loss \(\mathcal{L}_{\text{rec}}\) and the two self-supervised losses \(\mathcal{L}_{\text{ssl1}}\) and \(\mathcal{L}_{\text{ssl2}}\), weighted by their respective hyperparameters:
\begin{equation}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{rec}} + \mu^{\text{train}}_1 \mathcal{L}_{\text{ssl1}} + \mu^{\text{train}}_2 \mathcal{L}_{\text{ssl2}},
\label{main_loss}
\end{equation}
where \(\mu^{\text{train}}_1\) and \(\mu^{\text{train}}_2\) are the weights for the self-supervised losses. This combined loss optimizes the model by integrating both the primary task and self-supervised learning objectives.

\subsubsection{Testing Process}
During testing, the pre-trained model parameters are adaptively fine-tuned on all test samples. For each batch of test data, optimization is performed using the self-supervised losses \(\mathcal{L}_{\text{ssl1}}\) and \(\mathcal{L}_{\text{ssl2}}\) as defined in Equation~(\ref{ssl1}) and Equation~(\ref{ssl2}). The trained model is then used to make the final item predictions. After completing the predictions, the adjusted parameters are discarded, and the model reverts to its original parameters to process the next batch of test samples. The pseudo-code for processing a single batch of test samples is illustrated in Algorithm~\ref{alg:test_time_training}.
% \SetKwInOut{Input}{Input} % 自定义不缩进的 Input
% \SetKwInOut{Output}{Output} % 自定义不缩进的 Output
% \SetNlSty{textbf}{}{}

==> sections/4.0_exp_tab.tex <==
\begin{table}[t]
\centering
\caption{Dataset Statistics.}
\label{sta}
\begin{tabular}{l|r|r|r}
\hline
\textbf{Dataset} & \textbf{ML-1M} & \textbf{Amazon} & \textbf{Zhihu-1M} \\ 
\hline
\#Users & 6,034 & 247,659 & 7,974\\
\#Items & 3,706 & 10,814 & 81,563\\
\#Interactions & 1,000,209 & 471,615 & 999,970\\
Avg. Length & 138.3 & 17.04 & 29.03 \\
Sparsity & 95.57\% & 98.78\% & 99.48\% \\
\hline
\end{tabular}
\end{table}

\begin{table*}[t]
\centering
  \caption{Performance Comparison of Different Sequential Recommendation Models. The best result is bolded and the runner-up is underlined. * means improvements over the second-best methods are significant (\textit{t}-test, \textit{p}-value < 0.05).}
  \label{tab:main}
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c}{ML-1M} & \multicolumn{3}{c}{Amazon} & \multicolumn{3}{c}{Zhihu-1M} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& Recall@10 & MRR@10 & NDCG@10 & Recall@10 & MRR@10 & NDCG@10 & Recall@10 & MRR@10 & NDCG@10  \\
\hline
\hline
Caser & $0.1954$ & $0.0703$ & $0.0994$ & $0.0594$ & $0.0204$ & $0.0294$ & $0.0288$ & $0.0089$ & $0.0134$\\
GRU4Rec & $0.2732$ & $0.1147$ & $0.1518$ & $0.0939$ & $0.0480$ & $0.0586$ & $0.0283$ & $0.0092$ & $0.0142$\\
BERT4Rec & $0.2770$ & $0.1093$ & $0.1482$ & $0.0675$ & $0.0372$ & $0.0443$ & $0.0289$ & $0.0098$ & $0.0142$\\
SASRec & $0.2471$ & $0.0911$ & $0.1273$ & $\underline{0.1025}$ & $0.0527$ & $0.0644$ & $0.0364$ & $0.0098$ & $0.0159$ \\
% Mamba4Rec & $0.2950$ & $0.1274$ & $0.1665$ & $0.1020$ & $0.0546$ & $0.0657$ & $0.0409$ & $0.0133$ & $0.0197$\\
Mamba4Rec & $0.2813$ & $0.1201$ & $0.1578$ & $0.1003$ & $0.0522$ & $0.0635$ & $0.0355$ & $0.0112$ & $0.0167$\\
TiM4Rec & $0.2873$ & $\underline{0.1211}$ & $0.1596$ & $0.1016$ & $\underline{0.0567}$ & $\underline{0.0665}$ & \underline{$0.0384$} & \underline{$0.0118$} & \underline{$0.0179$}\\
TTT4Rec & $\underline{0.2887}$ & ${0.1208}$ & $\underline{0.1599}$ & $0.1020$ & $0.0560$ & $0.0655$ & $0.0370$ & $0.0115$ & $0.0174$\\
\ourname & $\mathbf{0.2984}$ & $\mathbf{0.1247}$ &$\mathbf{0.1651}$ & $\mathbf{0.1102}$ & $\mathbf{0.0580}$ & $\mathbf{0.0705}$ & $\mathbf{0.0402}$ & $\mathbf{0.0122}$ & $\mathbf{0.0187}$\\
\hline
\end{tabular}
\end{table*}



==> sections/4_exp.tex <==
\section{Experiments}
\input{sections/4.0_exp_tab}
To verify the effectiveness of \ourname, we conduct extensive experiments and report detailed analysis results.

\subsection{Experimental Settings}
\subsubsection{Datasets}
We evaluate the performance of the proposed model through experiments conducted on three public datasets:
\begin{itemize}[leftmargin=*]
    \item MovieLens-1M (referred to as \textbf{ML-1M})~\cite{harper2015movielens}: A dataset collected from the MovieLens platform, containing approximately 1 million user ratings of movies.
    \item Amazon Prime Pantry (referred to as \textbf{Amazon})~\cite{ni2019justifying}: A dataset of user reviews in the grocery category collected from the Amazon platform up to 2018.
    \item \textbf{Zhihu-1M}~\cite{hao2021large}: A dataset sourced from a large knowledge-sharing platform (Zhihu), consisting of raw data, including information on questions, answers, and user profiles.
\end{itemize}
For each user, we sort their interaction records by timestamp to generate an interaction sequence for each individual. 
% Following the methodology established in previous research~\cite{kang2018self}, we retain only users and items associated with at least five interaction records.
We retain only users and items associated with at least ten interaction records.
We follow the leave-one-out policy~\cite{kang2018self} for training-validation-testing partition. The statistical details of these datasets are presented in Table~\ref{sta}.

\subsubsection{Baselines}
To demonstrate the effectiveness of our proposed method, we conduct comparisons with several representative sequential recommendation baseline models:
\begin{itemize}[leftmargin=*]
    \item \textbf{Caser}~\cite{tang2018personalized}: A foundational sequential recommendation model leveraging Convolutional Neural Networks (CNN).
    \item \textbf{GRU4Rec}~\cite{hidasi2015session}: A method based on Recurrent Neural Networks (RNN), specifically utilizing Gated Recurrent Units (GRU) for sequential recommendation.
    \item \textbf{BERT4Rec}~\cite{sun2019bert4rec}: A sequential recommendation model that adopts the bidirectional attention mechanism inspired by the BERT~\cite{devlin2018bert} framework.
    \item \textbf{SASRec}~\cite{kang2018self}: The first model to introduce the Transformer architecture to the field of sequential recommendation.
    \item \textbf{Mamba4Rec}~\cite{liu2024mamba4rec}: An innovative model that applies the Mamba architecture to the sequential recommendation domain.
    % \item \textbf{SSD4Rec}~\cite{qu2024ssd4rec}: The first sequential recommendation model to utilize the SSD architecture, leveraging its superiority over traditional SSM approaches for high-dimensional data.
    \item \textbf{TiM4Rec}~\cite{fan2024tim4rec}: A time-aware sequential recommendation model that improves SSD's low-dimensional performance while maintaining computational efficiency.
    \item \textbf{TTT4Rec}~\cite{yang2024ttt4rec}: A framework that uses Test-Time Training to dynamically adapt model parameters during inference for sequential recommendation.
\end{itemize}
\subsubsection{Evaluation Metrics}
To evaluate the performance of top-$K$ recommendation, we adopt the metrics Recall@$K$, MRR@$K$, and NDCG@$K$, which are widely used in recommendation research to evaluate model performance~\cite{qu2024scalable, zhang2024qagcf, qu2024budgeted}. In this context, we set $K = 10$ and present the average scores on the test dataset.
\subsubsection{Implementation Details}
Our evaluation is based on implementations using PyTorch~\cite{paszke2019pytorch} and RecBole~\cite{zhao2021recbole}. We set all model dimensions $d$ to $64$, the learning rate to $0.001$, and the batch size to $4096$. Additionally, we set the state dimension $d_s$ of the \ourblockname\ to $32$, the number of blocks to $1$, the training steps M during testing $M$ to $1$ and learning rate during testing $\alpha$ to $0.005$. Furthermore, the search space for the weights of the two self-supervised losses during training, $\lambda^{\text{train}}_1$ and $\lambda^{\text{train}}_2$, is $\{0.01, 0.1, 1, 10\}$, and for testing, the search space for $\lambda^{\text{test}}_1$ and $\lambda^{\text{test}}_2$ is $\{1e-5, 1e-4, 1e-3, 1e-2, 1e-1\}$. To adapt to the characteristics of the baselines and datasets, we set the fixed sequence length to 200 for ML-1M and 50 for other datasets (Amazon and Zhihu-1M). For a fair comparison, we ensured consistency of key hyperparameters across different models while using default hyperparameters for baseline methods as recommended in their respective papers. Finally, we utilized the Adam optimizer~\cite{kingma2014adam} in a mini-batch training manner.

\subsection{Overall Performance}
Table~\ref{tab:main} presents the performance comparison of the proposed \ourname\ and other baseline methods on three datasets. From the table, we observe several key insights:
\begin{enumerate}[leftmargin=*]
    \item General sequential methods, such as SASRec and Mamba4Rec, show varying strengths depending on the dataset characteristics. Mamba4Rec performs better on ML-1M, a dataset with longer sequences, due to its ability to model complex long-term dependencies, whereas SASRec achieves slightly higher performance on shorter sequence datasets like Amazon and Zhihu-1M, where simpler sequence modeling suffices.
    \item TiM4Rec and TTT4Rec outperform these general sequential methods by addressing specific challenges in recommendation. Tim4Rec effectively incorporates temporal information, enhancing its ability to model time-sensitive dynamics, while TTT4Rec leverages test-time training to address distribution shifts, leading to superior performance.
    \item Finally, \ourname\ outperforms all baselines across datasets, achieving the best results by introducing time interval alignment loss and \oursslname\ alignment loss. These innovations enable \ourname\ to capture temporal and sequential patterns more effectively and adapt dynamically to test data through gradient descent during inference, further addressing distributional shifts and enhancing overall performance.
\end{enumerate}
\begin{table*}[t]
\centering
  \caption{Ablation Studies.}
  \label{tab:ablation}
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c}{ML-1M} & \multicolumn{3}{c}{Amazon} & \multicolumn{3}{c}{Zhihu-1M} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& Recall@10 & MRR@10 & NDCG@10 & Recall@10 & MRR@10 & NDCG@10 & Recall@10 & MRR@10 & NDCG@10  \\
\hline
\hline
\ourname & $0.2984$ & $0.1247$ & $0.1651$ & $0.1102$ & $0.0580$ & $0.0705$ & $0.0402$ & $0.0122$ & $0.0187$\\
\hdashline
w/o SSL & $0.2813$ & $0.1207$ & $0.1578$ & $0.1003$ & $0.0522$ & $0.0635$ & $0.0355$ & $0.0112$ & $0.0167$\\
w/o SSL$_1$ & $0.2891$ & $0.1225$ & $0.1618$ & $0.1076$ & $0.0571$ & $0.0689$ & $0.0389$ & $0.0118$ & $0.0182$\\
w/o SSL$_2$ & $0.2910$ & $0.1214$ & $0.1603$ & $0.1010$ & $0.0545$ & $0.0652$ & $0.0365$ & $0.0114$ & $0.0175$\\
\hdashline
w/o TTT & $0.2949$ & $0.1228$ & $0.1628$ & $0.1090$ & $0.0572$ & $0.0700$ & $0.0395$ & $0.0120$ & $0.0184$\\
w/o TTT$_1$ & $0.2977$ & $0.1253$ & $0.1643$ & $0.1095$ & $0.0575$ & $0.0702$ & $0.0400$ & $0.0122$ & $0.0185$\\
w/o TTT$_2$ & $0.2965$ & $0.1242$ & $0.1641$ & $0.1100$ & $0.0578$ & $0.0704$ & $0.0397$ & $0.0120$ & $0.0188$\\
\hline
\end{tabular}
\end{table*}

\begin{table}[t]
\centering
  \caption{Analysis of Test-Time Throughput.}
  \label{tab:timeana}
\begin{tabular}{l|c|c|c}
\hline
\multirow{2}{*}{Model} & \multicolumn{1}{c}{ML-1M} & \multicolumn{1}{c}{Amazon} & \multicolumn{1}{c}{Zhihu-1M} \\
\cline{2-4}
& \multicolumn{3}{c}{Test-Time Throughput (it/s)}\\
\hline
\hline
SASRec & $1.56$ & $2.26$ & $1.96$  \\
Mamba4Rec & $2.82$ & $3.11$ & $3.01$ \\
TiM4Rec & $2.16$ & $2.64$ & $2.56$ \\
TTT4Rec & $0.96$ & $1.74$ & $1.19$ \\
\ourname & $1.02$ & $2.05$ &$1.36$ \\
\hline
\end{tabular}
\end{table}

\subsection{Ablation Studies}
We conducted ablation experiments in \ourname\ to validate the effectiveness of the self-supervised losses we designed: time interval alignment loss and \oursslname\ alignment loss. Specifically, the configurations `w/o SSL', `w/o SSL$_1$' and `w/o SSL$_2$' represent models where we removed both self-supervised losses, only the time interval alignment loss, and only the \oursslname\ alignment loss during training, respectively. Additionally, we designed the `w/o TTT', `w/o TTT$_1$', and `w/o TTT$_2$' configurations, where all self-supervised losses are retained during training but not applied during testing, or where only one self-supervised loss is applied during testing. These experiments were conducted with the same parameter settings and training processes, except for the removal of the corresponding self-supervised losses.

The results shown in Table~\ref{tab:ablation} indicate that removing any of the self-supervised losses leads to a significant performance drop, with the `w/o SSL' configuration, where both losses were removed, resulting in the largest decline. This highlights the critical importance of both losses for the model's overall effectiveness. Furthermore, the configurations `w/o TTT', `w/o TTT$_1$', and `w/o TTT$_2$' show that not adapting to the test data using self-supervised losses during testing negatively impacts performance. This further emphasizes the importance of performing adaptive adjustments during testing to address distribution shifts in recommender systems.

We provide a deeper analysis of these results as follows: (1) The time interval alignment loss helps the model learn temporal dependencies, enabling it to better handle time-varying patterns during testing. (2) The \oursslname\ alignment loss aids in capturing and maintaining the inherent structure of state transitions, helping the model adapt to recommendation patterns in the system, and thereby enhancing robustness. (3) By reintroducing self-supervised losses during testing to adapt to the current data’s temporal and recommendation patterns, the model's performance is further improved. This demonstrates that self-supervised losses are not only important during training but also crucial during testing to address distribution shift issues and optimize model performance.

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{fig/ana1.pdf}
\caption{Sensitivity Analysis of $\mu_1^{\text{train}}$ and $\mu_2^{\text{train}}$.}
\label{ana1}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{fig/ana2.pdf}
\caption{Sensitivity Analysis of $\mu_1^{\text{test}}$ and $\mu_2^{\text{test}}$.}
\label{ana2}
\end{figure}


\subsection{Further Analysis}
% \subsubsection{Analysis under Different Data Split Ratios}
% To fully exploit the potential of \ourname, we considered replacing the leave-one-out method with other data splitting strategies. Since our focus is on test-time training, which primarily takes effect during the testing phase, we aim to include more test data. Specifically, we followed the setting in~\cite{yang2024ttt4rec} to split the dataset based on timestamps, using ratios of [$0.6$, $0.2$, $0.2$] and [$0.3$, $0.2$, $0.5$]. The results are presented in Table~\ref{tab:split622} and Table~\ref{tab:split325}. As shown in the results, our method achieved a more significant performance improvement compared to the leave-one-out approach. This demonstrates the effectiveness of \ourname\ in achieving adaptation during the testing phase.
% \subsubsection{Analysis of Distribution Shifts}
\subsubsection{Analysis of Test-time Throughput}
Noticed that training during testing requires gradient descent, which could introduce additional load on test-time (inference) throughput. To address this, we conducted offline experiments to analyze the impact of training during testing. The results are shown in Table~\ref{tab:timeana}, where we compare \ourname\ with several typical baselines and quantify the test-time throughput in terms of it/s (iterations per second). From the results in the table, it is evident that the test-time throughput of the method that trains during testing is approximately half of that of Mamba4Rec that does not train during testing. Nevertheless, with increasing computational power, the additional load from training during testing may not have a significant impact, especially since previous work has shown that TTT has yielded online benefits~\cite{wang2024not}. We present these findings and provide optimization opportunities for future work applying TTT in recommendations.

\subsubsection{Sensitive Analysis of $\mu_1^{\text{train}}$ and $\mu_2^{\text{train}}$}
We analyze the impact of the two self-supervised loss weight parameters, $\mu_1^{\text{train}}$ and $\mu_2^{\text{train}}$, in the training process of Equation~\ref{main_loss} in \ourname\ as shown in Figure~\ref{ana1}.
$\mu_1^{\text{train}}$ is the weight of the time interval alignment loss during training, while $\mu_2^{\text{train}}$ is the weight of the \oursslname\ alignment loss during training. The smaller the value of $\mu_1^{\text{train}}$ and $\mu_2^{\text{train}}$, the less influence each loss has on the model training.
From Figure~\ref{ana1}, we observe that the optimal choice for $\mu_1^{\text{train}}$ is $0.1$ and for $\mu_2^{\text{train}}$ is $1$. It is clear that both losses significantly impact the training of \ourname, with the \oursslname\ alignment loss having a slightly greater effect. This also confirms the importance of the model understanding the current recommendation pattern.

\subsubsection{Sensitive Analysis of $\mu_1^{\mathrm{test}}$ and $\mu_2^{\mathrm{test}}$}
We analyze the impact of the two self-supervised loss weight parameters, $\mu_1^{\text{test}}$ and $\mu_2^{\text{test}}$, during the testing process of \ourname. 
$\mu_1^{\text{test}}$ is the weight of the time interval alignment loss during testing, while $\mu_2^{\text{test}}$ is the weight of the \oursslname\ alignment loss during testing. The smaller the values of $\mu_1^{\text{test}}$ and $\mu_2^{\text{test}}$, the less impact each loss has on the model during testing.
From Figure~\ref{ana2}, we observe that the optimal choice for $\mu_1^{\text{test}}$ is $1e-5$, and for $\mu_2^{\text{test}}$ it is $1e-2$. It is clear that the \oursslname\ alignment loss has a significant impact on the model's performance during testing. The model needs to correctly learn the current recommendation pattern from the input sequence and adapt accordingly to make better next-time predictions for the user.


\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{fig/ana3.pdf}
\caption{Analysis of Inference Batch Size.}
\label{ana3}
\end{figure}

\subsubsection{Analysis of Inference Batch Size}
We analyzed the impact of different batch sizes during testing on the final results. The motivation behind this analysis is that our model performs gradient descent separately for each batch of test data to adapt. Theoretically, different batch sizes should have different effects on the final outcome, because different test data may follow different distributions. Grouping test data with significantly different distributions together for Test-Time Training could lead to unstable effects. The final analysis results are shown in Figure~\ref{ana3}. As seen, when the batch size is $256$ and $1024$, Recall@$10$ and NDCG@$10$ reaches its highest value, indicating that performing gradient descent on samples with different batch sizes can achieve varying adaptation effects. However, regardless of this, reducing the batch size increases the testing time, and the differences brought by varying batch sizes on the final results are not significant. Therefore, in all the experiments presented in this paper, we performed Test-Time Training on the entire test dataset. 

Additionally, another meaningful direction for future research is the batching strategy for test data. Grouping test data that follows the same distribution within a single batch for Test-Time Training could provide further insights, and this aspect is left for future exploration.

==> sections/5_conclusion.tex <==
\section{Conclusion and Future Work}
In this work, we addressed the critical challenge of adapting sequential recommendation to real-world scenarios where user interest shifts dynamically at the test time. Existing methods, reliant on static training data, often fail to adapt effectively to these changes, leading to substantial performance degradation. To overcome this limitation, we introduced \ourname, a novel approach that integrates Test-Time Training (TTT) into sequential recommendation through two alignment-based self-supervised losses. By aligning absolute time intervals with model-adaptive learning intervals and incorporating a state alignment mechanism, \ourname\ captures temporal dynamics and user interest patterns more effectively. Extensive evaluations on multiple benchmark datasets demonstrate that \ourname\ significantly outperforms existing methods, providing robust performance and mitigating the effects of distribution shifts. This work highlights the potential of TTT as a paradigm for enhancing the adaptability of sequential recommendation at the test time.

As a future research direction, the focus should first be on the efficiency of applying Test-Time Training in recommendations. Existing work has mainly applied TTT in the re-ranking phase~\cite{wang2024not}, but optimizing TTT for broader applications within recommendations remains an area that requires further exploration. Additionally, the batching strategy for TTT during the testing phase is another issue that needs attention. How to batch test data more effectively based on prior data distributions for optimized gradient descent is a promising research direction, which warrants further investigation in future studies.
